Video DataFlywheel: Resolving the Impossible Data Trinity in Video-Language Understanding

Recently, video-language understanding has achieved great success through large-scale pre-training. However, data scarcity remains a prevailing challenge. This study quantitatively reveals an "impossible trinity" among data quantity, diversity, and quality in pre-training datasets. Recent efforts seek to refine large-scale, diverse ASR datasets compromised by low quality through synthetic annotations. These methods successfully leverage useful information in multimodal video content (frames, tags, ASR transcripts, etc.) to refine the original annotations. Nevertheless, they struggle to mitigate noise within synthetic annotations and lack scalability as the dataset size expands. To address these issues, we introduce the Video DataFlywheel framework, which iteratively refines video annotations with improved noise control methods. For iterative refinement, we first leverage a video-language model to generate synthetic annotations, resulting in a refined dataset. Then, we pre-train on it and fine-tune on human refinement examples for a stronger model. These processes are repeated for continuous improvement. For noise control, we present AdaTaiLr, a novel noise control method that requires weaker assumptions on noise distribution, thereby proving more effective in large datasets with theoretical guarantees. The combination of iterative refinement and AdaTaiLr can achieve better scalability in video-language understanding. Extensive experiments show that our framework outperforms existing data refinement baselines, delivering a 3% performance boost and improving dataset quality with minimal diversity loss. Furthermore, our refined dataset facilitates significant improvements in various video-language understanding tasks, including video question answering and text-video retrieval.

==> bibli.tex <==
%---------------- (1) video-language datasets ------------------%
@inproceedings{miech_howto100m_2019,
    title = {{HowTo100M}: {Learning} a {Text}-{Video} {Embedding} by {Watching} {Hundred} {Million} {Narrated} {Video} {Clips}},
    booktitle = {Proceedings of the {International} {Conference} on {Computer} {Vision}},
    publisher = {IEEE},
    author = {Miech, Antoine and Zhukov, Dimitri and Alayrac, Jean-Baptiste and Tapaswi, Makarand and Laptev, Ivan and Sivic, Josef},
    year = {2019},
    pages = {2630--2640}
}

@inproceedings{zellers_yt-tmp-180m_2021,
    title = {{MERLOT}: {Multimodal} {Neural} {Script} {Knowledge} {Models}},
    booktitle = {Proceedings of the Advances in {Neural} {Information} {Processing} {Systems}},
    author = {Zellers, Rowan and Lu, Ximing and Hessel, Jack and Yu, Youngjae and Park, Jae Sung and Cao, Jize and Farhadi, Ali and Choi, Yejin},
    year = {2021},
    pages = {23634--23651},
    publisher = {Neural Information Processing Systems Foundation},
}


@inproceedings{zellers_yt-tmp-2b_2022,
	title = {{MERLOT} {RESERVE}: {Neural} {Script} {Knowledge} through {Vision} and {Language} and {Sound}},
	booktitle = {Proceedings of the {Conference} on {Computer} {Vision} and {Pattern} {Recognition}},
	publisher = {IEEE},
	author = {Zellers, Rowan and Lu, Jiasen and Lu, Ximing and Yu, Youngjae and Zhao, Yanpeng and Salehi, Mohammadreza and Kusupati, Aditya and Hessel, Jack and Farhadi, Ali and Choi, Yejin},
	year = {2022},
	pages = {16354--16366},
}


@inproceedings{xue_hd-vila_2022,
  author       = {Hongwei Xue and
                  Tiankai Hang and
                  Yanhong Zeng and
                  Yuchong Sun and
                  Bei Liu and
                  Huan Yang and
                  Jianlong Fu and
                  Baining Guo},
  title        = {Advancing High-Resolution Video-Language Representation with Large-Scale
                  Video Transcriptions},
  booktitle    = {Proceedings of the Conference on Computer Vision and Pattern Recognition},
  pages        = {5026--5035},
  publisher    = {{IEEE}},
  year         = {2022}
}

@inproceedings{bain_webvid_2021,
    title = {Frozen in {Time}: {A} {Joint} {Video} and {Image} {Encoder} for {End}-to-{End} {Retrieval}},
    booktitle = {Proceedings of the {International} {Conference} on {Computer} {Vision}},
    publisher = {IEEE},
    author = {Bain, Max and Nagrani, Arsha and Varol, Gül and Zisserman, Andrew},
    year = {2021},
    pages = {1708--1718},
}

@inproceedings{msrvtt_2016,
  author       = {Jun Xu and
                  Tao Mei and
                  Ting Yao and
                  Yong Rui},
  title        = {{MSR-VTT:} {A} {Large} {Video} {Description} {Dataset} for {Bridging} {Video}
                  and {Language}},
  booktitle    = {Proceedings of the Conference on Computer Vision and Pattern Recognition},
  pages        = {5288--5296},
  publisher    = {{IEEE} Computer Society},
  year         = {2016},
}

@inproceedings{msvd_2011,
	title = {Collecting {Highly} {Parallel} {Data} for {Paraphrase} {Evaluation}},
	booktitle = {Proceedings of the {Annual} {Meeting} of the {Association} for {Computational} {Linguistics}: {Human} {Language} {Technologies}},
	publisher = {The Association for Computer Linguistics},
	author = {Chen, David L. and Dolan, William B.},
	year = {2011},
	pages = {190--200},
}

@inproceedings{vatex_2019,
	title = {{VaTeX}: {A} {Large}-{Scale}, {High}-{Quality} {Multilingual} {Dataset} for {Video}-and-{Language} {Research}},
	booktitle = {Proceedings of the {International} {Conference} on {Computer} {Vision}},
	publisher = {IEEE},
	author = {Wang, Xin and Wu, Jiawei and Chen, Junkun and Li, Lei and Wang, Yuan-Fang and Wang, William Yang},
	year = {2019},
	pages = {4580--4590},
}

@inproceedings{anet_caption_2017,
	title = {Dense-{Captioning} {Events} in {Videos}},
	booktitle = {Proceedings of the {International} {Conference} on {Computer} {Vision}},
	publisher = {IEEE Computer Society},
	author = {Krishna, Ranjay and Hata, Kenji and Ren, Frederic and Fei-Fei, Li and Niebles, Juan Carlos},
	year = {2017},
	pages = {706--715},
}


@inproceedings{hendricks_didemo_2017,
	title = {Localizing {Moments} in {Video} with {Natural} {Language}},
	booktitle = {Proceedings of the {International} {Conference} on {Computer} {Vision}},
	publisher = {IEEE Computer Society},
	author = {Hendricks, Lisa Anne and Wang, Oliver and Shechtman, Eli and Sivic, Josef and Darrell, Trevor and Russell, Bryan C.},
	year = {2017},
	pages = {5804--5813},
}


@inproceedings{youcook_2016,
  author       = {Luowei Zhou and
                  Chenliang Xu and
                  Jason J. Corso},
  title        = {Towards Automatic Learning of Procedures From Web Instructional Videos},
  booktitle    = {Proceedings of the {AAAI} Conference on Artificial Intelligence},
  pages        = {7590--7598},
  publisher    = {{AAAI} Press},
  year         = {2018}
}

@inproceedings{qvhighlights_2021,
	title = {{Detecting} {Moments} and {Highlights} in {Videos} via {Natural} {Language} {Queries}},
	volume = {34},
	booktitle = {Proceedings of the Advances in {Neural} {Information} {Processing} {Systems}},
	author = {Lei, Jie and Berg, Tamara L and Bansal, Mohit},
	year = {2021},
        publisher = {Neural Information Processing Systems Foundation},
}



@misc{luo_valley_2023,
	title = {Valley: {Video} {Assistant} with {Large} {Language} model {Enhanced} {abilitY}},
	author = {Luo, Ruipu and Zhao, Ziwang and Yang, Min and Dong, Junwei and Li, Da and Lu, Pengcheng and Wang, Tao and Hu, Linmei and Qiu, Minghui and Wei, Zhongyu},
	year = {2023},
	note = {arXiv:2306.07207 [cs]},
}




%---------------- (2) vision-language dataset refinement ------------------%
@inproceedings{miech_mil_nce_2020,
	title = {End-to-{End} {Learning} of {Visual} {Representations} {From} {Uncurated} {Instructional} {Videos}},
	booktitle = {Proceedings of the {Conference} on {Computer} {Vision} and {Pattern} {Recognition}},
	publisher = {Computer Vision Foundation / IEEE},
	author = {Miech, Antoine and Alayrac, Jean-Baptiste and Smaira, Lucas and Laptev, Ivan and Sivic, Josef and Zisserman, Andrew},
	year = {2020},
	pages = {9876--9886},
}

@inproceedings{huang_ncr_2021,
	title = {Learning with {Noisy} {Correspondence} for {Cross}-modal {Matching}},
	booktitle = {Proceedings of the Advances in {Neural} {Information} {Processing} {Systems}},
        publisher = {Neural Information Processing Systems Foundation},
	author = {Huang, Zhenyu and Niu, Guocheng and Liu, Xiao and Ding, Wenbiao and Xiao, Xinyan and Wu, Hua and Peng, Xi},
	year = {2021},
	pages = {29406--29419},
}

@article{yang_just_ask_2022,
	title = {Learning to {Answer} {Visual} {Questions} from {Web} {Videos}},
	urldate = {2023-11-30},
	journal = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
	author = {Yang, Antoine and Miech, Antoine and Sivic, Josef and Laptev, Ivan and Schmid, Cordelia},
	year = {2022},
	pages = {1--12},
}

@inproceedings{li_blip_2022,
	title = {{BLIP}: {Bootstrapping} {Language}-{Image} {Pre}-training for {Unified} {Vision}-{Language} {Understanding} and {Generation}},
	booktitle = {Proceedings of the International {Conference} on {Machine} {Learning}},
	publisher = {PMLR},
	author = {Li, Junnan and Li, Dongxu and Xiong, Caiming and Hoi, Steven C. H.},
	year = {2022},
	pages = {12888--12900},
}

@inproceedings{li_blip2_2023,
  author       = {Junnan Li and
                  Dongxu Li and
                  Silvio Savarese and
                  Steven C. H. Hoi},
  title        = {{BLIP-2:} Bootstrapping Language-Image Pre-training with Frozen Image
                  Encoders and Large Language Models},
  booktitle    = {International Conference on Machine Learning, {ICML}},
  series       = {Proceedings of Machine Learning Research},
  pages        = {19730--19742},
  publisher    = {{PMLR}},
  year         = {2023}
}

@article{betker_dali3_2023,
  title={Improving image generation with better captions},
  author={Betker, James and Goh, Gabriel and Jing, Li and Brooks, Tim and Wang, Jianfeng and Li, Linjie and Ouyang, Long and Zhuang, Juntang and Lee, Joyce and Guo, Yufei and others},
  journal={Computer Science. https://cdn. openai. com/papers/dall-e-3. pdf},
  volume={2},
  pages={8},
  year={2023}
}

@inproceedings{fan_laclip_2023,
	title = {Improving {CLIP} {Training} with {Language} {Rewrites}},
	booktitle = {Proceedings of the Advances in {Neural} {Information} {Processing} {Systems}},
	author = {Fan, Lijie and Krishnan, Dilip and Isola, Phillip and Katabi, Dina and Tian, Yonglong},
	year = {2023},
        publisher = {Neural Information Processing Systems Foundation},
}

@inproceedings{nguyen_improving_2023,
	title = {{Improving} {Multimodal} {Datasets} with {Image} {Captioning}},
	booktitle = {Proceedings of the Advances in {Neural} {Information} {Processing} {Systems}},
	author = {Nguyen, Thao and Gadre, Samir Yitzhak and Ilharco, Gabriel and Oh, Sewoong and Schmidt, Ludwig},
	year = {2023},
}

@article{feng_ctpr_2023,
	title = {Learning {From} {Noisy} {Correspondence} {With} {Tri}-{Partition} for {Cross}-{Modal} {Matching}},
	journal = {IEEE Transactions on Multimedia},
	author = {Feng, Zerun and Zeng, Zhimin and Guo, Caili and Li, Zheng and Hu, Lin},
	year = {2023},
        volume={26},
	pages = {1--14},
}

@inproceedings{xue_clip_vip_2023,
	title = {{CLIP}-{ViP}: {Adapting} {Pre}-trained {Image}-{Text} {Model} to {Video}-{Language} {Representation} {Alignment}},
	author = {Xue, Hongwei and Sun, Yuchong and Liu, Bei and Fu, Jianlong and Song, Ruihua and Li, Houqiang and Luo, Jiebo},
	year = {2023},
        booktitle = {Proceedings of the {International} {Conference} on {Learning} {Representations}},
	publisher = {OpenReview.net},
        pages = {1--8}
}

@inproceedings{chen_vast_2023,
	title = {{VAST}: {A} {Vision}-{Audio}-{Subtitle}-{Text} {Omni}-{Modality} {Foundation} {Model} and {Dataset}},
	booktitle = {Proceedings of the Advances in {Neural} {Information} {Processing} {Systems}},
	author = {Chen, Sihan and Li, Handong and Wang, Qunbo and Zhao, Zijia and Sun, Mingzhen and Zhu, Xinxin and Liu, Jing},
	year = {2023},
        pages = {1--8},
        publisher = {Neural Information Processing Systems Foundation}
}

@inproceedings{chen_panda_70m_2024,
	title = {Panda-70m: {Captioning} 70m videos with multiple cross-modality teachers},
	booktitle = {Proceedings of the {Conference} on {Computer} {Vision} and {Pattern} {Recognition}},
	author = {Chen, Tsai-Shien and Siarohin, Aliaksandr and Menapace, Willi and Deyneka, Ekaterina and Chao, Hsiang-wei and Jeon, Byung Eun and Fang, Yuwei and Lee, Hsin-Ying and Ren, Jian and Yang, Ming-Hsuan and {others}},
	year = {2024},
	pages = {13320--13331},
        publisher = {Computer Vision Foundation / IEEE},
}

@inproceedings{wang_internvid_2023,
	title = {{InternVid}: {A} {Large}-scale {Video}-{Text} {Dataset} for {Multimodal} {Understanding} and {Generation}},
	author = {Wang, Yi and He, Yinan and Li, Yizhuo and Li, Kunchang and Yu, Jiashuo and Ma, Xin and Chen, Xinyuan and Wang, Yaohui and Luo, Ping and Liu, Ziwei and Wang, Yali and Wang, Limin and Qiao, Yu},
	year = {2023},
        booktitle = {Proceedings of the {International} {Conference} on {Learning} {Representations}},
	publisher = {OpenReview.net},
        pages = {1--8}
}

@inproceedings{lai_veclip_2024,
	title = {{VeCLIP}: {Improving} {CLIP} {Training} via {Visual}-enriched {Captions}},
	author = {Lai, Zhengfeng and Zhang, Haotian and Zhang, Bowen and Wu, Wentao and Bai, Haoping and Timofeev, Aleksei and Du, Xianzhi and Gan, Zhe and Shan, Jiulong and Chuah, Chen-Nee and Yang, Yinfei and Cao, Meng},
	year = {2024},
        booktitle = {Proceedings of the {European} {Conference} on {Computer} {Vision}},
        pages = {13320--13331},
        publisher = {Computer Vision Foundation / IEEE},
}




%---------------- (3) VideoLLM models ------------------%
@inproceedings{moviechat,
	title = {{MovieChat}: {From} {Dense} {Token} to {Sparse} {Memory} for {Long} {Video} {Understanding}},
	author = {Song, Enxin and Chai, Wenhao and Wang, Guanhong and Zhang, Yucheng and Zhou, Haoyang and Wu, Feiyang and Chi, Haozhe and Guo, Xun and Ye, Tian and Zhang, Yanting and Lu, Yan and Hwang, Jenq-Neng and Wang, Gaoang},
	booktitle = {Proceedings of the {Conference} on {Computer} {Vision} and {Pattern} {Recognition}},
	publisher = {Computer Vision Foundation / IEEE},
        pages = {9876--9886},
	year = {2024},
}

@article{llama_vid,
  title = {{LLaMA}-{VID}: {An} {Image} is {Worth} 2 {Tokens} in {Large} {Language} {Models}},
  author={Li, Yanwei and Wang, Chengyao and Jia, Jiaya},
  journal={arXiv preprint arXiv:2311.17043},
  year={2023}
}

@article{video_llava,
    title = {Video-{LLaVA}: {Learning} {United} {Visual} {Representation} by {Alignment} {Before} {Projection}},
    author={Lin, Bin and Zhu, Bin and Ye, Yang and Ning, Munan and Jin, Peng and Yuan, Li},
    journal={arXiv preprint arXiv:2311.10122},
    year={2023}
}

@inproceedings{videochat2,
	title = {{MVBench}: {A} {Comprehensive} {Multi}-modal {Video} {Understanding} {Benchmark}},
	author = {Li, Kunchang and Wang, Yali and He, Yinan and Li, Yizhuo and Wang, Yi and Liu, Yi and Wang, Zun and Xu, Jilan and Chen, Guo and Luo, Ping and Wang, Limin and Qiao, Yu},
	booktitle = {Proceedings of the {Conference} on {Computer} {Vision} and {Pattern} {Recognition}},
	publisher = {Computer Vision Foundation / IEEE},
        pages = {718–731},
	year = {2024},
}

@misc{llava_next,
  title={{LLaVA}-{NeXT}: A {Strong} {Zero}-{shot} {Video} {Understanding} {Model}},
  url={https://llava-vl.github.io/blog/2024-04-30-llava-next-video/},
  author={Zhang, Yuanhan and Li, Bo and Liu, haotian and Lee, Yong jae and Gui, Liangke and Fu, Di and Feng, Jiashi and Liu, Ziwei and Li, Chunyuan},
  month={April},
  year={2024}
}

@inproceedings{video_llama_2023,
	title = {Video-{LLaMA}: {An} {Instruction}-tuned {Audio}-{Visual} {Language} {Model} for {Video} {Understanding}},
	booktitle = {Proceedings of the {Conference} on {Empirical} {Methods} in {Natural} {Language} {Processing}},
	publisher = {Association for Computational Linguistics},
	author = {Zhang, Hang and Li, Xin and Bing, Lidong},
	year = {2023},
	pages = {543--553},
}

@article{videochat_2023,
  title = {{VideoChat}: {Chat}-{Centric} {Video} {Understanding}},
  author={Li, KunChang and He, Yinan and Wang, Yi and Li, Yizhuo and Wang, Wenhai and Luo, Ping and Wang, Yali and Wang, Limin and Qiao, Yu},
  journal={arXiv preprint arXiv:2305.06355},
  year={2023}
}

@misc{videococa_2023,
	title = {{VideoCoCa}: {Video}-{Text} {Modeling} with {Zero}-{Shot} {Transfer} from {Contrastive} {Captioners}},
	author = {Yan, Shen and Zhu, Tao and Wang, Zirui and Cao, Yuan and Zhang, Mi and Ghosh, Soham and Wu, Yonghui and Yu, Jiahui},
	year = {2023},
	note = {arXiv:2212.04979 [cs]}
}

@misc{chat_univi_2023,
	title = {Chat-{UniVi}: {Unified} {Visual} {Representation} {Empowers} {Large} {Language} {Models} with {Image} and {Video} {Understanding}},
	publisher = {arXiv},
	author = {Jin, Peng and Takanobu, Ryuichi and Zhang, Caiwan and Cao, Xiaochun and Yuan, Li},
	year = {2023},
	note = {arXiv:2311.08046 [cs]}
}

@inproceedings{video_chatgpt_2023,
    title = {Video-{ChatGPT}: {Towards} {Detailed} {Video} {Understanding} via {Large} {Vision} and {Language} {Models}},
    author={Maaz, Muhammad and Rasheed, Hanoona and Khan, Salman and Khan, Fahad Shahbaz},
    booktitle = {Proceedings of the Annual Meeting of the Association for Computational Linguistics},
    publisher = {Association for Computational Linguistics},
    pages = {1--12},
    year = {2024},
}


@inproceedings{yang_frozenbilm_2022,
	title = {Zero-{Shot} {Video} {Question} {Answering} via {Frozen} {Bidirectional} {Language} {Models}},
	booktitle = {Proceedings of the Advances in {Neural} {Information} {Processing} {Systems}},
	author = {Yang, Antoine and Miech, Antoine and Sivic, Josef and Laptev, Ivan and Schmid, Cordelia},
	year = {2022},
        publisher = {Neural Information Processing Systems Foundation},
}


@article{zhang_llama_adapter_2023,
	title = {{LLaMA}-{Adapter}: {Efficient} {Fine}-tuning of {Language} {Models} with {Zero}-init {Attention}},
	volume = {abs/2303.16199},
	author = {Zhang, Renrui and Han, Jiaming and Zhou, Aojun and Hu, Xiangfei and Yan, Shilin and Lu, Pan and Li, Hongsheng and Gao, Peng and Qiao, Yu},
	year = {2023},
	note = {arXiv: 2303.16199},
}


@article{ma_vista_llama_2023,
	title = {Vista-{LLaMA}: {Reliable} {Video} {Narrator} via {Equal} {Distance} to {Visual} {Tokens}},
	author = {Ma, Fan and Jin, Xiaojie and Wang, Heng and Xian, Yuchen and Feng, Jiashi and Yang, Yi},
	year = {2023},
	note = {arXiv: 2312.08870},
}


@article{lita_2024,
  author       = {De{-}An Huang and
                  Shijia Liao and
                  Subhashree Radhakrishnan and
                  Hongxu Yin and
                  Pavlo Molchanov and
                  Zhiding Yu and
                  Jan Kautz},
  title        = {{LITA:} Language Instructed Temporal-Localization Assistant},
  volume       = {abs/2403.19046},
  year         = {2024},
  eprinttype    = {arXiv},
}


@article{st_llm_2024,
  author       = {Ruyang Liu and
                  Chen Li and
                  Haoran Tang and
                  Yixiao Ge and
                  Ying Shan and
                  Ge Li},
  title        = {{ST-LLM:} Large Language Models Are Effective Temporal Learners},
  volume       = {abs/2404.00308},
  year         = {2024},
  eprinttype    = {arXiv},
}


@misc{xu_pllava_2024,
	title = {{PLLaVA} : {Parameter}-free {LLaVA} {Extension} from {Images} to {Videos} for {Video} {Dense} {Captioning}},
	publisher = {arXiv},
	author = {Xu, Lin and Zhao, Yilin and Zhou, Daquan and Lin, Zhijie and Ng, See Kiong and Feng, Jiashi},
	year = {2024},
	note = {arXiv:2404.16994 [cs]}
}



@misc{kim_ig_vlm_2024,
	title = {An {Image} {Grid} {Can} {Be} {Worth} a {Video}: {Zero}-shot {Video} {Question} {Answering} {Using} a {VLM}},
	publisher = {arXiv},
	author = {Kim, Wonkyun and Choi, Changin and Lee, Wonseok and Rhee, Wonjong},
	year = {2024},
	note = {arXiv:2403.18406 [cs]},
}




%---------------- (4) TaiLr related ------------------%
@inproceedings{tailr,
	title = {Tailoring {Language} {Generation} {Models} under {Total} {Variation} {Distance}},
	booktitle = {Proceedings of the {International} {Conference} on {Learning} {Representations}},
	publisher = {OpenReview.net},
	author = {Ji, Haozhe and Ke, Pei and Hu, Zhipeng and Zhang, Rongsheng and Huang, Minlie},
	year = {2023},
        pages = {1-8}
}

@inproceedings{loss_truncation,
	title = {Improved {Natural} {Language} {Generation} via {Loss} {Truncation}},
	booktitle = {Proceedings of the {Annual} {Meeting} of the {Association} for {Computational} {Linguistics}},
	publisher = {Association for Computational Linguistics},
	author = {Kang, Daniel and Hashimoto, Tatsunori B.},
	year = {2020},
	pages = {718--731},
}

@inproceedings{gold,
  author       = {Richard Yuanzhe Pang and
                  He He},
  title        = {Text Generation by Learning from Demonstrations},
  booktitle    = {Proceedings of the {International} {Conference} on {Learning} {Representations}},
  publisher    = {OpenReview.net},
  year         = {2021},
  pages = {88-96}
}

@article{tvd_textbook,
  title={Probability in high dimension},
  author={Van Handel, Ramon},
  journal={Lecture Notes (Princeton University)},
  year={2014}
}

@book{ESL,
  title={The elements of statistical learning: data mining, inference, and prediction},
  author={Hastie, Trevor and Tibshirani, Robert and Friedman, Jerome H and Friedman, Jerome H},
  volume={2},
  year={2009},
  publisher={Springer}
}


@inproceedings{li_ENT_2023,
	title = {Error {Norm} {Truncation}: {Robust} {Training} in the {Presence} of {Data} {Noise} for {Text} {Generation} {Models}},
	author = {Li, Tianjian and Xu, Haoran and Koehn, Philipp and Khashabi, Daniel and Murray, Kenton},
	year = {2024},
        booktitle = {Proceedings of the {International} {Conference} on {Learning} {Representations}},
	publisher = {OpenReview.net},
        pages = {1--8}
}





%---------------- (5) Others ------------------%
@inproceedings{liu_llava_2023,
    title = {Visual {Instruction} {Tuning}},
    booktitle = {Proceedings of the Advances in {Neural} {Information} {Processing} {Systems}},
    author = {Liu, Haotian and Li, Chunyuan and Wu, Qingyang and Lee, Yong Jae},
    year = {2023},
    publisher = {Neural Information Processing Systems Foundation},
}

@inproceedings{vicuna_llm,
  author       = {Lianmin Zheng and
                  Wei{-}Lin Chiang and
                  Ying Sheng and
                  Siyuan Zhuang and
                  Zhanghao Wu and
                  Yonghao Zhuang and
                  Zi Lin and
                  Zhuohan Li and
                  Dacheng Li and
                  Eric P. Xing and
                  Hao Zhang and
                  Joseph E. Gonzalez and
                  Ion Stoica},
  title        = {{Judging} {LLM}-as-a-Judge with {MT}-Bench and {Chatbot} {Arena}},
  booktitle    = {Proceedings of the Advances in Neural Information Processing Systems},
  year         = {2023}
}

@inproceedings{clip_2021,
	title = {Learning {Transferable} {Visual} {Models} {From} {Natural} {Language} {Supervision}},
	booktitle = {Proceedings of the {International} {Conference} on {Machine} {Learning}},
	publisher = {PMLR},
	author = {Radford, Alec and Kim, Jong Wook and Hallacy, Chris and Ramesh, Aditya and Goh, Gabriel and Agarwal, Sandhini and Sastry, Girish and Askell, Amanda and Mishkin, Pamela and Clark, Jack and Krueger, Gretchen and Sutskever, Ilya},
	year = {2021},
	pages = {8748--8763}
}

@inproceedings{xu_msrvttmsvdqa_2017,
  title={Video question answering via gradually refined attention over appearance and motion},
  author={Xu, Dejing and Zhao, Zhou and Xiao, Jun and Wu, Fei and Zhang, Hanwang and He, Xiangnan and Zhuang, Yueting},
  booktitle={Proceedings of the {International} {Conference} on {Multimedia}},
  publisher = {ACM},
  pages={1645--1653},
  year={2017}
}

@inproceedings{yu_anetqa_2019,
  title={Activitynet-qa: A dataset for understanding complex web videos via question answering},
  author={Yu, Zhou and Xu, Dejing and Yu, Jun and Yu, Ting and Zhao, Zhou and Zhuang, Yueting and Tao, Dacheng},
  booktitle={Proceedings of the {AAAI} {Conference} on {Artificial} {Intelligence}},
  publisher = {AAAI Press},
  pages={9127--9134},
  year={2019}
}

@inproceedings{li_tgifqa_2016,
  author       = {Yuncheng Li and
                  Yale Song and
                  Liangliang Cao and
                  Joel R. Tetreault and
                  Larry Goldberg and
                  Alejandro Jaimes and
                  Jiebo Luo},
  title        = {{TGIF:} {A} New Dataset and Benchmark on Animated {GIF} Description},
  booktitle    = {Proceedings of the {Conference} on {Computer} {Vision} and {Pattern} {Recognition}},
  pages        = {4641--4650},
  publisher    = {{IEEE} Computer Society},
  year         = {2016}
}


@inproceedings{vedantam_cider_2015,
	title = {{CIDEr}: {Consensus}-based image description evaluation},
	booktitle = {Proceedings of the {Conference} on {Computer} {Vision} and {Pattern} {Recognition}},
	publisher = {IEEE Computer Society},
	author = {Vedantam, Ramakrishna and Zitnick, C. Lawrence and Parikh, Devi},
	year = {2015},
	pages = {4566--4575},
}


@inproceedings{bertasius_timesformer_2021,
	title = {Is {Space}-{Time} {Attention} {All} {You} {Need} for {Video} {Understanding}?},
	booktitle = {Proceedings of the {International} {Conference} on {Machine} {Learning}},
	publisher = {PMLR},
	author = {Bertasius, Gedas and Wang, Heng and Torresani, Lorenzo},
	year = {2021},
	pages = {813--824}
}


@inproceedings{li_umt_2023,
	title = {Unmasked {Teacher}: {Towards} {Training}-{Efficient} {Video} {Foundation} {Models}},
	booktitle = {Proceedings of the {International} {Conference} on {Computer} {Vision}},
	publisher = {IEEE},
	author = {Li, Kunchang and Wang, Yali and Li, Yizhuo and Wang, Yi and He, Yinan and Wang, Limin and Qiao, Yu},
	year = {2023},
	pages = {19891--19903}
}


@inproceedings{wang_omnivl_2022,
	title = {{OmniVL}: {One} {Foundation} {Model} for {Image}-{Language} and {Video}-{Language} {Tasks}},
	booktitle = {Proceedings of the Advances in {Neural} {Information} {Processing} {Systems}},
	author = {Wang, Junke and Chen, Dongdong and Wu, Zuxuan and Luo, Chong and Zhou, Luowei and Zhao, Yucheng and Xie, Yujia and Liu, Ce and Jiang, Yu-Gang and Yuan, Lu},
	year = {2022}
}


@inproceedings{cheng_vindlu_2023,
	title = {{VindLU}: {A} {Recipe} for {Effective} {Video}-and-{Language} {Pretraining}},
	booktitle = {Proceedings of the {Conference} on {Computer} {Vision} and {Pattern} {Recognition}},
	publisher = {IEEE},
	author = {Cheng, Feng and Wang, Xizi and Lei, Jie and Crandall, David J. and Bansal, Mohit and Bertasius, Gedas},
	year = {2023},
	pages = {10739--10750}
}


@inproceedings{xue_clip-vip_2023,
	title = {{CLIP}-{ViP}: {Adapting} {Pre}-trained {Image}-{Text} {Model} to {Video}-{Language} {Alignment}},
	booktitle = {Proceedings of the {International} {Conference} on {Learning} {Representations}},
	publisher = {OpenReview.net},
	author = {Xue, Hongwei and Sun, Yuchong and Liu, Bei and Fu, Jianlong and Song, Ruihua and Li, Houqiang and Luo, Jiebo},
	year = {2023},
	pages = {1--12}
}

@inproceedings{guan_pidro_2023,
  title={Pidro: Parallel isomeric attention with dynamic routing for text-video retrieval},
  author={Guan, Peiyan and Pei, Renjing and Shao, Bin and Liu, Jianzhuang and Li, Weimian and Gu, Jiaxi and Xu, Hang and Xu, Songcen and Yan, Youliang and Lam, Edmund Y},
  booktitle={Proceedings of the International Conference on Computer Vision},
  publisher = {IEEE},
  pages={11164--11173},
  year={2023}
}

@inproceedings{wang_rtq_2023,
  title={RTQ: Rethinking Video-language Understanding Based on Image-text Model},
  author={Wang, Xiao and Li, Yaoyu and Gan, Tian and Zhang, Zheng and Lv, Jingjing and Nie, Liqiang},
  booktitle={Proceedings of the International Conference on Multimedia},
  pages={557--566},
  year={2023},
  publisher = {ACM},
}

@article{internvideo_2022,
  title={{Internvideo}: {General} {Video} {Foundation} {Models} via {Generative} and {Discriminative} {Learning}},
  author={Wang, Yi and Li, Kunchang and Li, Yizhuo and He, Yinan and Huang, Bingkun and Zhao, Zhiyu and Zhang, Hongjie and Xu, Jilan and Liu, Yi and Wang, Zun and others},
  journal={arXiv preprint arXiv:2212.03191},
  year={2022}
}



@inproceedings{guo_animatediff_2023,
	title = {{AnimateDiff}: {Animate} {Your} {Personalized} {Text}-to-{Image} {Diffusion} {Models} without {Specific} {Tuning}},
	author = {Guo, Yuwei and Yang, Ceyuan and Rao, Anyi and Wang, Yaohui and Qiao, Yu and Lin, Dahua and Dai, Bo},
	year = {2024},
        booktitle = {Proceedings of the {International} {Conference} on {Learning} {Representations}},
        publisher = {OpenReview.net},
        pages = {1--8}
}

@misc{ucf101,
  author       = {Khurram Soomro and
                  Amir Roshan Zamir and
                  Mubarak Shah},
  title        = {{UCF101:} {A} Dataset of 101 Human Actions Classes From Videos in The Wild},
  volume       = {abs/1212.0402},
  year         = {2012},
  eprinttype    = {arXiv},
}

@article{mu_embodiedgpt_2024,
  title={Embodiedgpt: Vision-language pre-training via embodied chain of thought},
  author={Mu, Yao and Zhang, Qinglong and Hu, Mengkang and Wang, Wenhai and Ding,       Mingyu and Jin, Jun and Wang, Bin and Dai, Jifeng and Qiao, Yu and Luo, Ping},
  journal={Proceedings of the {Advances} in {Neural} {Information} {Processing} {Systems}},
  volume={36},
  publisher = {OpenReview.net},
  year={2024}
}

@inproceedings{dong_m2paap_2024,
  title={M2-RAAP: A Multi-Modal Recipe for Advancing Adaptation-based Pre-training towards Effective and Efficient Zero-shot Video-text Retrieval},
  author={Dong, Xingning and Feng, Zipeng and Zhou, Chunluan, and Yu, Xuzheng and Yang, Ming and Guo, Qingpei},
  booktitle={Proceedings of the {International} SIGIR {Conference} on {Research} and {Development} in {Information} {Retrieval}},
  pages={2156--2166},
  year={2024}
}

@article{luo_clip4clip_2022,
  title={Clip4clip: An empirical study of clip for end to end video clip retrieval and captioning},
  author={Luo, Huaishao and Ji, Lei and Zhong, Ming and Chen, Yang and Lei, Wen and Duan, Nan and Li, Tianrui},
  journal={Neurocomputing},
  volume={508},
  pages={293--304},
  year={2022},
  publisher={Elsevier}
}

@inproceedings{bertasius_timesformer_2021,
  title={Is space-time attention all you need for video understanding?},
  author={Bertasius, Gedas and Wang, Heng and Torresani, Lorenzo},
  booktitle={Proceedings of the ICML},
  pages={4},
  year={2021},
  publisher = {PMLR},
}

==> deprecated_parts/failed_theorem2.tex <==
\begin{restatable}[Approximation of Optimal $\gamma$]{theorem}{aog}
\label{thm:aog}
Given one-hot distribution sampled from real data $e^{(w)}\sim p_o^{<t}$, then the following function:
\begin{equation}
    \tilde{\Gamma}_{opt}(p_o^{<t}, p_\theta^{<t})=\frac{1}{2} + \lambda \left (
        \mathcal{L}_{\textmd{TVD}}(e^{(w)}, p_\theta^{<t}) - 2H_2(p_\theta^{<t})
    \right ),
\end{equation}
achieves the following approximation guarantee towards $\Gamma_{opt}$.
\begin{multline}
    \left |  
        \epsilon(p_o^{<t}, p_\theta^{<t}, \tilde{\Gamma}_{opt}) - \epsilon(p_o^{<t}, p_\theta^{<t}, \Gamma_{opt})
    \right | \\
    \le
    \frac{1}{16\lambda}
    +
    2 \left \| p_\theta^{<t} - p_o^{<t} \right \|_\infty
    +
    \delta,
\end{multline}
where $\delta=
\frac{1}{2} \mathbb{E}_{w\sim p_o} \left [ \left
    \| p_o^{<t} - e^{(w)}
\right \|_1 \right ]
$.
\end{restatable}
The full proof is presented in \autoref{sec:proof_aog}. 


% === Proof of approximation of optimal gamma ====================================================================
\subsection{Proof of Theorem~\ref{thm:aog}} \label{sec:proof_aog}

Before the proof, we will introduce how we approximate the $\Gamma_{opt}$, followed by some lemmas. We first use function $f(x)$ as the smooth approximation to the indicator function $\mathbbm{1}[x]$:
\begin{equation}
    f(x) = \begin{cases}
        0 & \text{ if } x < -\frac{1}{2\lambda} \\
        \lambda x + \frac{1}{2}   & \text{ if } -\frac{1}{2\lambda} \le x \le \frac{1}{2\lambda} \\
        1 & \text{ if } x > \frac{1}{2\lambda}
    \end{cases},
\end{equation}
where $\lambda>0$ is a constant. Obviously, we have
\begin{equation}
    \mathbbm{1}[x] = \lim_{\lambda \to \infty} f(x).
\end{equation}

Denote $x=\mathcal{L}_{\textmd{TVD}}(p_o^{<t}, p_\theta^{<t}) - 2H_2(p_o^{<t})$, we then use the predicted distribution $p_\theta$ to approximate the real distribution $p_o$ within $x$:
$\Tilde{x}=\mathcal{L}_{\textmd{TVD}}(e^{(w)}, p_\theta^{<t}) - 2H_2(p_\theta^{<t})$. Finally, the optimal $\Gamma$ function and our approximation $\Tilde{\Gamma}$ can be written as:
\begin{equation}
    \begin{cases}
        \Gamma_{opt} &= \mathbbm{1}[x], \\
        \Tilde{\Gamma}_{opt} &= f(\Tilde{x}).
    \end{cases}
\end{equation}


\begin{lemma}[Error from Smooth Approximation]
\label{lem:error_smooth}
    When employing function $f(x)$ as a smooth approximation to the indicator function $\mathbbm{1}[x]$, the error can be characterized by the subsequent bound:
    \begin{equation}
        \left | \mathbbm{1}[x] - f(x) \right | | x | \le \frac{1}{16\lambda}.
    \end{equation}
\end{lemma}

\begin{proof}
    \begin{align}
        \left | \mathbbm{1}[x] - f(x) \right | | x | &= \begin{cases}
            0 & \text{ if } x > \frac{1}{2\lambda} \\
            \left ( \frac{1}{2} - \lambda x \right ) |x| & \text{ if } 0 \le x \le \frac{1}{2\lambda} \\
            \left ( \frac{1}{2} + \lambda x \right ) |x| & \text{ if } -\frac{1}{2\lambda} \le x \le 0 \\
            0 & \text{ if } x < -\frac{1}{2\lambda}
        \end{cases} \\
        &= \begin{cases}
            0 & \text{ if } |x| > \frac{1}{2\lambda} \\
            \left ( \frac{1}{2} - \lambda |x| \right ) |x| & \text{ if } |x| \le \frac{1}{2\lambda} \\
        \end{cases} \\
        &\le \left ( \frac{1}{2} - \lambda |x| \right ) |x| \\
        &= -\lambda \left ( x - \frac{1}{4\lambda} \right )^2 + \frac{1}{16\lambda} \\
        &\le \frac{1}{16\lambda}
    \end{align}
\end{proof}


\begin{lemma}[Error from Real Distribution Approximation]
    \label{lem:error_distribution}
    When employing predicted distribution $p_\theta$ as an approximation to real data distribution $p_o$, the error can be characterized by the subsequent bound:
    \begin{multline}
        \mathbb{E}_{w\sim p_o} \left [ \left | f(x) - f(\Tilde{x}) \right | | x | \right ] \\
        \le 
        \frac{1}{2} \mathbb{E}_{w\sim p_o} \left [ \left
            \| p_o^{<t} - e^{(w)}
        \right \|_1 \right ]
        +
        2 \left \| p_\theta^{<t} - p_o^{<t} \right \|_\infty.
    \end{multline}
\end{lemma}

\begin{proof}
    We first prove three useful bounds. 
    
    The first is the upper bound of $| x |$. Since $\mathcal{L}_{\textmd{TVD}}(p_o^{<t}, p_\theta^{<t})\in[0, 1]$ and 
    $2H_2(p_o^{<t})\in[0,1]$, 
    \begin{equation}
        | x | = \left | \mathcal{L}_{\textmd{TVD}}(p_o^{<t}, p_\theta^{<t}) - 2H_2(p_o^{<t}) \right | \le 1.
    \end{equation}
    The second is the upper bound of the approximation error for TVD :
    \begin{align}
        & \mathbb{E}_{w\sim p_o} \left [ \left | \mathcal{L}_{\textmd{TVD}}(p_o^{<t}, p_\theta^{<t}) 
              - \mathcal{L}_{\textmd{TVD}}(e^{(w)}, p_\theta^{<t}) \right | \right ] \\
        &= \frac{1}{2} \mathbb{E}_{w\sim p_o} \left [ \left | 
                \| p_o^{<t} - p_\theta^{<t} \|_1 - \| e^{(w)} - p_\theta^{<t} \|_1
            \right | \right ] \\
        &= \frac{1}{2} \mathbb{E}_{w\sim p_o} \left [ \left | 
                \| p_o^{<t} - p_\theta^{<t} \|_1 - \| p_\theta^{<t} - e^{(w)} \|_1
            \right | \right ] \\
        &\le \frac{1}{2} \mathbb{E}_{w\sim p_o} \left [ \left
                \| \left ( p_o^{<t} - p_\theta^{<t} \right ) + \left ( p_\theta^{<t} - e^{(w)} \right )
            \right \|_1 \right ] \\
        &= \frac{1}{2} \mathbb{E}_{w\sim p_o} \left [ \left
                \| p_o^{<t} - e^{(w)}
            \right \|_1 \right ].
    \end{align}
    The third is the upper bound of the approximation error for Tsallis 2-entropy:
    \begin{align}
        & \left | 2 H_2(p_o^{<t}) - 2H_2(p_\theta^{<t}) \right | \\
        &= \left | \sum_{i}\left [ \left( p_{\theta i}^{<t} \right)^2 - \left( p_{oi}^{<t} \right)^2 \right ] \right | \\
        &\le \sum_{i}\left | \left( p_{\theta i}^{<t} \right)^2 - \left( p_{oi}^{<t} \right)^2 \right | \\
        &= \sum_{i}\left | \left( p_{\theta i}^{<t} + p_{oi}^{<t} \right) \left( p_{\theta i}^{<t} - p_{oi}^{<t} \right) \right | \label{eq:proof_holderleft} \\
        &\le \left \| p_\theta^{<t} + p_o^{<t} \right \|_1 \left \| p_\theta^{<t} - p_o^{<t} \right \|_\infty \label{eq:proof_holderright} \\
        &= 2 \left \| p_\theta^{<t} - p_o^{<t} \right \|_\infty.
    \end{align}
    From \autoref{eq:proof_holderleft} to \autoref{eq:proof_holderright} we use the Hölder's inequality:
    \begin{equation}
        \left \| \mathbf{u}\odot\mathbf{v} \right \|_1 \le \left \| \mathbf{u} \right \|_p \left \| \mathbf{v} \right \|_q, \frac{1}{p} + \frac{1}{q} = 1,
    \end{equation}
    where $\mathbf{u},\mathbf{v}$ are vectors, $p,q\in[1, \infty]$, and $\odot$ means pointwise product between two vectors.

    Finally, we can prove the lemma:
    \begin{align}
        & \mathbb{E}_{w\sim p_o} \left [ \left | f(x) - f(\Tilde{x}) \right | | x | \right ] \\
        &\le \mathbb{E}_{w\sim p_o} \left [ \left | f(x) - f(\Tilde{x}) \right | \right ] \\
        &= \mathbb{E}_{w\sim p_o} [ | \mathcal{L}_{\textmd{TVD}}(p_o^{<t}, p_\theta^{<t}) 
              - \mathcal{L}_{\textmd{TVD}}(e^{(w)}, p_\theta^{<t}) \\
            &\quad - 2 \left ( H_2(p_o^{<t}) - H_2(p_\theta^{<t}) \right )
            | ] \\
        &\le \mathbb{E}_{w\sim p_o} \left [ \left | \mathcal{L}_{\textmd{TVD}}(p_o^{<t}, p_\theta^{<t}) 
              - \mathcal{L}_{\textmd{TVD}}(e^{(w)}, p_\theta^{<t}) \right | \right ] \\
              &\quad  +  \mathbb{E}_{w\sim p_o} \left [ \left | 2 H_2(p_o^{<t}) - 2H_2(p_\theta^{<t}) \right | \right ] \\
        &\le \frac{1}{2} \mathbb{E}_{w\sim p_o} \left [ \left
                \| p_o^{<t} - e^{(w)}
            \right \|_1 \right ]
            +
            2 \left \| p_\theta^{<t} - p_o^{<t} \right \|_\infty.
    \end{align}
\end{proof}


\aog*

\begin{proof}
The approximation error can be written as:
\begin{align} 
    &\left |  
        \epsilon(p_o^{<t}, p_\theta^{<t}, \tilde{\Gamma}_{opt}) - \epsilon(p_o^{<t}, p_\theta^{<t}, \Gamma_{opt})
    \right | \\
    &= \left | \left ( {\Gamma_{opt} - \Tilde{\Gamma}_{opt}} \right ) x \right | \\
    &= \left | \mathbbm{1}[x] - f(\Tilde{x}) \right | | x | \\
    &= \left | \mathbbm{1}[x] - f(x) + f(x) - f(\Tilde{x}) \right | | x | \\
    &\le \left | \mathbbm{1}[x] - f(x) \right | | x | + \left | f(x) - f(\Tilde{x}) \right | | x | \\
    &\le \frac{1}{16\lambda} + \frac{1}{2} \mathbb{E}_{w\sim p_o} \left [ \left
        \| p_o^{<t} - e^{(w)}
    \right \|_1 \right ]
    +
    2 \left \| p_\theta^{<t} - p_o^{<t} \right \|_\infty.
\end{align}
In the last step, we adopt Lemma \autoref{lem:error_smooth} and Lemma \autoref{lem:error_distribution}.


\end{proof}

==> parts/IV_part_videogen.tex <==
\subsection{Text-to-Video Generation}


\subsubsection{Experimental Settings}

\textbf{Model, training datasets, and implementation details.}
To evaluate the effectiveness of text-to-video generation, we use AnimateDiff \cite{guo_animatediff_2023} as the base model trained on our 2.5M randomly sampled video-text pairs. We follow the implementation details in their official codebase. During training, we fix image-to-text modules and only train the motion modeling modules. For each training video, we sample 16 frames with a stride of 4, and then resize and center-crop to 256 × 256 resolution.


\textbf{Evaluation datasets and metrics.} 
Downstream datasets and evaluation metrics. To evaluate the models, we follow the evaluation protocols \cite{chen_panda_70m_2024, wang_internvid_2023} for zero-shot evaluation on UCF101 \cite{ucf101} and MSR-VTT \cite{msrvtt_2016}. Specifically, we generate 16-frame videos in 256 × 256px resolution. For UCF101, we produce a text prompt for each class and generate 10,000 videos that share the same class distribution as the original dataset. We compute Fréchet Video Distance (FVD) on the I3D embeddings. 
%
For MSRVTT, we generate a video sample for each of the 59,800 test prompts and compute CLIP similarity (CLIPSim).

% We also show the generated video samples in Figure 6. To visualize the results, we follow the official codebase and replace SDT2I with personalized Dreambooth weight [60], TUSUN3. Note that the test prompt and the video sample from the AnimtateDiff with the official weight (top row in Figure 6) are directly from the project page of AnimateDiff.


\subsubsection{Performance Comparison}

\input{tables/videogen_results}


As illustrated in \autoref{tab:videogen_results}, VidDataFlyWheel-2M pretraining consistently shows superior performance on both metrics compared to the other refined datasets. 
% As highlighted, our pretraining yields 77.4 lower FVD on UCF101 and outperforms state-of-the-art models pre-trained on a dataset within a 10M scale in terms of FVD. 
% Qualitatively, our pretraining weights can generate the video with a more meaningful motion and photorealistic appearance and do not include a watermark.

==> tables/videogen_results.tex <==
\begin{table}[t]

\caption{
Performance comparison in text-to-video generation benchmark.
}

\centering
\label{tab:videogen_results}
\resizebox{\linewidth}{!}{


\begin{tabular}{ccccc}
\hline
\multirow{2}{*}{Method} & \multirow{2}{*}{Training Data} & UCF101 &  & MSR-VTT \\ \cline{3-3} \cline{5-5} 
                        &                                & FVD    &  & CLIPSIM \\ \hline
VideoCrafter            & WebVid10M                      & 910.9  &  & 0.2875  \\
VideoFusion             & WebVid10M                      & 639.9  &  & 0.2795  \\
InternVid-t2v           & WebVid10M                      & 705.3  &  & 0.2657  \\
InternVid-t2v           & WebVid10M+InternVid18M         & 616.5  &  & 0.2951  \\
AnimateDiff             & WebVid2.5M                     & 499.3  &  & 0.2869  \\
AnimateDiff             & Panda2M                        & 421.9  &  & 0.2880  \\ \hline
AnimateDiff             & Ours2M                         & 418.4  &  & 0.2912  \\ \hline
\end{tabular}


}
\end{table}
